Self-Supervised Open-Ended Classification with Small Visual Language Models

We present Self-Context Adaptation (SeCAt), a self-supervised approach that unlocks few-shot abilities for open-ended classification with small visual language models. Our approach imitates image captions in a self-supervised way based on clustering a large pool of images followed by assigning semantically-unrelated names to clusters. By doing so, we construct a training signal consisting of interleaved sequences of image and pseudocaption pairs and a query image, which we denote as the 'self-context' sequence. Based on this signal the model is trained to produce the right pseudo-caption. We demonstrate the performance and flexibility of SeCAt on several multimodal few-shot datasets, spanning various granularities. By using models with approximately 1B parameters we outperform the few-shot abilities of much larger models, such as Frozen and FROMAGe. SeCAt opens new possibilities for research and applications in open-ended few-shot learning that otherwise requires access to large or proprietary models.

==> tables/abl_clustering.tex <==
% \begin{table}[t]
\centering
  \caption{
  Self-supervised clustering vs noisy supervision.
  }
  \label{tab:ablation_self_supervised}
  \centering
    %\resizebox{1\columnwidth}{!}{\setlength\tabcolsep{4pt}
    \begin{tabular}{cccccc}
    \toprule
    & \multicolumn{2}{c}{\textbf{2-way}} & \multicolumn{2}{c}{\textbf{5-way}} \\
    \cmidrule(lr){2-3} \cmidrule(lr){4-6}
        self-sup? & 1-shot & 5-shot  & 1-shot & 5-shot \\
        \midrule
         \xmark & 76.9 &  73.7  & 55.2 & 50.2 &\\
        \cmark & \textbf{85.7} & \textbf{83.2}  & \textbf{68.6} & \textbf{58}  \\
    \bottomrule
  \end{tabular}

% \end{table}

 %%%%%%%%%% old version below

%  \begin{table}[t]
% \small
%   \caption{
%   Benefit of performing the clustering step as a way to learn a self-context is measured on the Real-Name miniImageNet dataset.
%   }
%   \vspace{-2mm}
%   \label{tab:ablation_clustering}
%   \centering
%     \resizebox{1\columnwidth}{!}{\setlength\tabcolsep{4pt}
%     \begin{tabular}{lccccccc}
%     \toprule
%     & & \multicolumn{3}{c}{\textbf{2-way miniImageNet}} & \multicolumn{3}{c}{\textbf{5-way miniImageNet}} \\
%     \cmidrule(lr){3-5} \cmidrule(lr){6-8}
%         Method & self-supervision? & 1-shot & 3-shot & 5-shot & 1-shot & 3-shot & 5-shot \\
%         \midrule
%         \multirow{2}{*}{\textbf{SeCAt (Ours)}} & \xmark & 76.9 & 81.3 & 73.7 & 55.2 & &\\
%         & \cmark & \textbf{85.7} & \textbf{88.2} & \textbf{83.2} & \textbf{68.6} & \textbf{59.3} & \textbf{58} \\
%     \bottomrule
%   \end{tabular}
%   }
% \end{table}

==> tables/abl_num_clusters.tex <==

% |           			2-way  	        	| 	5-way  	        	|        	
% |-------------------	|--------	|--------	|--------	|--------	|--------	|--------	|
% | # clusters 	| 1-shot 	| 3-shot 	| 5-shot 	| 1-shot 	| 3-shot 	| 5-shot 	|
% |     25    	|   30.2	|  31.1	|   18.7	|   13.6	|   5.4	|   3.9	|
% |     50    	|   72.8	|  73.8	|   71.6	|   45.0	|  40.5	|  24.0	|
% |     75    	|   84.4	|  78.6	|   79.3	|  54.5	|  49.8	|  48.1	|
% |    100    	|   85.7	|  88.2	|  83.2	|  68.6	|  62.4 	|  58.0	|
% |    200    	|   83.1	|  83.1	|  65.1	|  59.6	|  49.9	|  45.9	|

\centering
  \caption{
  The number of $k$ clusters.
  }
  \label{tab:ablation_self_supervised}
  \centering
    %\resizebox{1\columnwidth}{!}{\setlength\tabcolsep{4pt}
    \begin{tabular}{cccccc}
    \toprule
    & \multicolumn{2}{c}{\textbf{2-way}} & \multicolumn{2}{c}{\textbf{5-way}} \\
    \cmidrule(lr){2-3} \cmidrule(lr){4-6}
        $k$ & 1-shot & 5-shot  & 1-shot & 5-shot \\
        \midrule
        25 & 30.2 & 18.7 & 13.6 & 3.9 &\\
        50  & 72.8 & 71.6  & 45.0 & 24.0 &\\
        75  & 84.4 & 79.3 &  54.5 & 48.1 &\\
        100  & 85.7 & 83.2 & 68.6 & 58.0 &\\
        200  & 83.1 & 65.1 & 59.6 & 45.9 &\\
    \bottomrule
  \end{tabular}

==> tables/abl_tightness.tex <==
% \begin{table}[t]
  \caption{
  Source cluster coherence.
  }
  % \vspace{-2mm}
  \label{tab:ablation_cluster_tightness}
  \centering
    % \resizebox{1\columnwidth}{!}{\setlength\tabcolsep{4pt}
    \begin{tabular}{ccccc}
    \toprule
    & \multicolumn{2}{c}{\textbf{2-way}} & \multicolumn{2}{c}{\textbf{5-way}} \\
    \cmidrule(lr){2-3} \cmidrule(lr){4-5}
      coherence & 1-shot & 5-shot & 1-shot & 5-shot  \\
        \midrule
         <5\%$^{\text{th}}$ perc.  & 73.7 & 82.1 & 45.6 & 35.4 \\
         >95\%$^{\text{th}}$ perc.  & \textbf{77.6} & \textbf{84.7} & \textbf{61.7} & \textbf{35.8}  \\
    \bottomrule
  \end{tabular}
% \end{table}

%% old below:

% \begin{table}[t]
% \small
%   \caption{
%   Comparison of different distances for the tightness of clusters, on the Real-Name miniImageNet dataset.
%   }
%   \vspace{-2mm}
%   \label{tab:ablation_tight_clusters}
%   \centering
%     \resizebox{\columnwidth}{!}{\setlength\tabcolsep{4pt}
%     \begin{tabular}{lccccccc}
%     \toprule
%     & & \multicolumn{3}{c}{\textbf{Real-Name 2-way miniImageNet}} & \multicolumn{3}{c}{\textbf{Real-Name 5-way miniImageNet}} \\
%     \cmidrule(lr){3-5} \cmidrule(lr){6-8}
%         Method & centroid max distance & 1-shot & 3-shot & 5-shot & 1-shot & 3-shot & 5-shot \\
%         \midrule
%         \multirow{2}{*}{\textbf{SeCAt (Ours)}} & 5  & - & - & - & - & - & - \\
%         & 10  & - & - & - & - & - & - \\
%     \bottomrule
%   \end{tabular}
%   }
% \end{table}
